Value-Based Massive Access through Goal-Oriented Irregular Repetition Slotted ALOHA

The goal-oriented communication paradigm is poised to enable novel real-time applications by easing the burden on communication networks while still delivering task-relevant information. However, efforts so far have focused on the encoding problem, while the design of medium access schemes is still in the early stages of development, especially when connectivity is to be provided to a massive number of devices, e.g., for remote monitoring. In this respect, existing goal-oriented approaches are often centralized or based on simplified underlying mechanisms, requiring unrealistic assumptions. In this work, we present the Goal-oriented Irregular Repetition Slotted ALOHA (GO-IRSA) scheme, which combines modern random access techniques with belief-based policies. GO-IRSA does not impose significant computing loads on the sensors or require frequent feedback, and it can reduce the average and worst-case error of the estimate of a distributed Wiener process by over 30% with respect to the optimal centralized solution in a network with thousands of sensors, and is robust to imperfect interference cancellation and inaccurate process knowledge.

==> fig/frame.tex <==
\begin{tikzpicture}[
  slot/.style={
    rectangle,
    draw,
    minimum height=0.8cm,
    text centered,
    font=\small\bfseries
  },
  dl/.style={slot, fill=blue!25, minimum width=0.8cm},
  ulong/.style={slot, fill=orange!35, minimum width=2.0cm},
  ul/.style={slot, fill=orange!35, minimum width=1.0cm},
  ack/.style={slot, fill=green!30, minimum width=1.8cm},
  frame/.style={slot, fill=gray!30, minimum width=1.8cm},
  brace label/.style={font=\footnotesize, midway, above=6pt}
]

%% --- Draw slots ---

% Frame
\node[frame, anchor=west] (f1) at (0,2) {Frame 1};
\node[frame, anchor=west] (f2) at (f1.east) {$\cdots$};
\node[frame, anchor=west] (fh) at (f2.east) {Frame H};


% DL slot 1
\node[dl] (dl1) at (0,0) {DL 1};

% DL slot 2
\node[dl, anchor=west] (dl2) at (dl1.east) {DL 2};

% UL
\node[ul, anchor=west] (ul1) at (dl2.east) {UL 1};
\node[ulong, anchor=west] (ulong) at (ul1.east) {$\cdots$};
\node[ul, anchor=west] (uln) at (ulong.east) {UL N};
\node[dl, anchor=west] (ack) at (uln.east) {ACK};

\draw[-] (f1.south west) -- (dl1.north west);
\draw[-] (f1.south east) -- (ack.north east);


\end{tikzpicture}
